Manas: Mining Software Repositories to Assist AutoML

Today deep learning is widely used for building software. A software engineering problem with deep learning is that finding an appropriate convolutional neural network (CNN) model for the task can be a challenge for developers. Recent work on AutoML, more precisely neural architecture search (NAS), embodied by tools like Auto-Keras aims to solve this problem by essentially viewing it as a search problem where the starting point is a default CNN model, and mutation of this CNN model allows exploration of the space of CNN models to find a CNN model that will work best for the problem. These works have had significant success in producing high-accuracy CNN models. There are two problems, however. First, NAS can be very costly, often taking several hours to complete. Second, CNN models produced by NAS can be very complex that makes it harder to understand them and costlier to train them. We propose a novel approach for NAS, where instead of starting from a default CNN model, the initial model is selected from a repository of models extracted from GitHub. The intuition being that developers solving a similar problem may have developed a better starting point compared to the default model. We also analyze common layer patterns of CNN models in the wild to understand changes that the developers make to improve their models. Our approach uses commonly occurring changes as mutation operators in NAS. We have extended Auto-Keras to implement our approach. Our evaluation using 8 top voted problems from Kaggle for tasks including image classification and image regression shows that given the same search time, without loss of accuracy, Manas produces models with 42.9% to 99.6% fewer number of parameters than Auto-Keras' models. Benchmarked on GPU, Manas' models train 30.3% to 641.6% faster than Auto-Keras' models.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.75.  \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.76.  Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.77.  Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.78.  Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.
	       

==> algorithms/adapt.tex <==
\begin{algorithm}
	\caption{\manas Apdaptation System}\label{alg:adapt}
	\begin{algorithmic}[1]
		\Procedure {adaptation}{layer}
		\State ANN $\gets$ list of dictionary
		\State layers $\gets$ list of layers
		\State optimizers $\gets$ list of optimizers
		
		\For {l $\in$ CNN}
		\If {getName(l) $\in$ layers}						
		\If  {Input Layer = True}
		\State addInputLayer(l, outputNode)	
		\ElsIf{$Onput Layer$ == True}
		\State addOutputLayer(l, outputNode)
		\Else
		\State addLayer(l, outputNode)	
		\EndIf
		
		
		\ElsIf{$getName(l)$ $\in$ $optimizers$}
		\State \hspace{12mm}addOptimizer(l)	
		\EndIf
		\EndFor
		\EndProcedure
		
	\end{algorithmic}
\end{algorithm}

==> algorithms/matching.tex <==
%\begin{algorithm}
%	\caption{Model Matching}
%	\label{algorithm:matching}
%	\begin{algorithmic}[1]
%		\State data $\gets$ List(model, [$\Delta$1, $\Delta$2])\label{alg:dist}
%		\State DNN\_cluster $\gets$ List() 
%		
%		\Procedure {model\_matching}{data}
%			\State DNN\_clustering(data)
%			\If  {size(DNN\_cluster) > $\delta$} 
%				\State DNN\_filtering(models)
%			\EndIf
%		\EndProcedure
%		\Procedure {DNN\_clustering}{data} \label{alg:lackstart}
%		\For {DNN $\in$ DNNs} 
%			\If {distances[0] = min1} 
%				\If {distances[1] = min2} 
%				
%					\State 	DNN\_cluster.append(DNN)
%				\Else
%					\State min2 $\gets$ distances[1]
%						\If {size(DNN\_cluster) < $\lambda$} 
%							\State DNN\_cluster.append(DNN) 
%						\EndIf
%				\EndIf
%			\Else
%				\State min1 $\gets$ distances[0]
%				\If {size(DNN\_cluster) < $\lambda$} 
%					\State DNN\_cluster.append(DNN) 	\label{alg:lackend}
%				\EndIf
%			\EndIf
%		\EndFor
%		\EndProcedure
%		\Procedure {DNN\_filtering}{data}
%			\State archt $\gets$ architecture\_equivalent(DNN\_cluster)
%			\For {DNN $\in$ DNN\_cluster}
%				\If {DNN\_archt(DNN) $\neq$  archt} 
%					\State DNN\_cluster.remove(DNN)
%				\EndIf
%			\EndFor
%		\EndProcedure		
%		\Procedure {architecture\_equivalent}{DNN\_cluster}
%			\State counter $\gets$ 0
%			\State common\_archt $\gets$ DNN\_archt(DNN\_cluster[0])
%			\For {DNN $\in$ DNN\_cluster} 
%				\State curr\_freq $\gets$ count(DNN\_archt(DNN))
%				\If {curr\_freq  > counter} 
%					\State counter $\gets$ currFreq 
%					\State common\_archt $\gets$ DNN\_archt(DNN)
%				\EndIf
%			\EndFor
%		\State \Return  common\_archt
%		\EndProcedure
%		\Procedure {DNN\_archt}{DNN}
%			\State archt $\gets$ List()
%			\For {layer $\in$ DNN}
%				\If {layer is convolutional or linear } 
%					\State (input, output) $\gets$ layer
%					\State archt.append(input, output)
%				\EndIf
%			\EndFor
%		\State \Return archt 
%		\EndProcedure		
%	\end{algorithmic}
%\end{algorithm}

\begin{algorithm}
	\caption{Model Clustering}
	\label{algorithm:matching}
	\begin{algorithmic}[1]
		\Procedure {Model\_Clustering}{data, models} \label{alg:lackstart}
		\State D $\gets$ []
		\For {m $\in$ models} 
		\State	$\Delta$i = $|$I1 - I2$|$
		\If {$\Delta$i == 0}
		\State	$\Delta$o = $|$O1 - O2$|$
		\State	$\Delta$s = 
		\State D.insert(($\Delta$o, $\Delta$s))
		\EndIf
		\EndFor
		
		\State clusters = G\_means(D)
		\For {c $\in$ clusters}
		\If {min(D) $\in$ c}
		\State cluster = c
		\State \textbf{break}
		\EndIf
		\EndFor
		
		\State \Return cluster 
		\EndProcedure		
	\end{algorithmic}
\end{algorithm}



%\begin{algorithm}
%	\caption{Model Matching}
%	\label{algorithm:matching}
%	\begin{algorithmic}[1]
%		\State $\textit{min1} \gets \text{0}$ 
%		\State $\textit{min2} \gets \text{0}$ 
%		\State $\textit{data} \gets \text{List of (model, [dist1, dist2])}$\label{alg:dist}
%		\State $\textit{models} \gets \text{List()}$ 
%		\State \textcolor{darkred}{\bf Procedure} {Len\_Check}(models)
%		\State	\hspace{4mm}  \textcolor{darkred}{\bf if} {$len(models)$ < $5$} \textcolor{darkred}{\bf then} 
%			\State \hspace{8mm} models.append(model)
%			
%		
%		
%		\Procedure{Extract\_Conv}{model}
%			\State $\textit{conv\_in\_out} \gets \text{List}$ 
%			\For {$layer$ $\in$ $model$}
%				\If {$layer$ $is$ $concolutional$ $layer$}
%					\State conv\_in\_out.append(input, output)
%				\EndIf
%			\EndFor
%			\State \Return conv\_in\_out
%		\EndProcedure
%
%		\Procedure{Architecture\_Equivalent}{models}
%			\State $\textit{counter} \gets \text{0}$
%			\State $\textit{conv\_in\_out} \gets \text{Extract\_Conv(models[0])}$
%			\For{$model$ $\in$ $models$}
%				\State {$curr\_freq$ = $count(Extract\_Conv(model))$}
%				\If {$curr\_freq$ > $counter$}
%					\State $\textit{counter} \gets \text{curr\_freq}$
%					\State $\textit{conv\_in\_out} \gets \text{Extract\_Conv(model)}$
%				\EndIf
%			\EndFor
%		\State \Return conv\_in\_out
%		\EndProcedure
%		
%		
%		\Procedure{Inadequate\_Model\_Matching}{data} \label{alg:lackstart}
%		\State $\textit{min1, min2} \gets \text{0, 0}$ 
%		%\State $\textit{min2} \gets \text{0}$ 
%		
%		\For{$model$, $distances$ $\in$ $data$}
%			\If {$distances[0]$ = $min1$}
%				\If {$distances[1]$ = $min2$}
%					\State $models.append(model)$
%				\Else
%					\State $min2 \gets distances[1]$
%					\State $Len\_Check(models)$
%				%						\Else
%				%						\State break
%				\EndIf
%				\Else
%					\State $min1 \gets distances[0]$
%					\State $Len\_Check(models)$	\label{alg:lackend}
%
%			\EndIf
%		\EndFor
%
%		\EndProcedure
%		
%		\Procedure{Redundant\_Model\_Matching}{data}
%			\State $\textit{architecture} \gets \text{Architecture\_Equivalent(models)}$ 
%			\For{$model$ $\in$ $models$}
%				\If {$Extract\_Conv(model)$ != $architecture$}
%					\State models.remove(model)
%				\EndIf
%			\EndFor
%		\EndProcedure
%		\Procedure{Model\_Selection}{data}
%		\State $\text{Inadequate\_Model\_Selection(data)}$ 
%		\If {$len(models)$ > $15$}
%			\State $Redundant\_Model\_Selection(models)$
%		\EndIf
%		\EndProcedure
%		
%	\end{algorithmic}
%\end{algorithm}


==> background/background.tex <==
\section{Background}
\subsection{Neural Architecture Search}
NAS \cite{elsken2018neural, wistuba2019survey} is a technique for automatically finding an apropriate machine learning (ML) model architecture which can outperform most of hand-made ML models. Specifically, NAS need only the training dataset as the input to create a powerful model architecture. There are many different approaches for a NAS system; however, most of them have three main components which are search space, search strategy, and optimization strategy.  

{\bf Search space.} The space represent the search boundary of a NAS system. In particular, the search space limit what kind of model architecture can be searched and optimizied. For instance, Baker \etal \cite{baker2016designing} use the convolutional architecture with pooling, linear transformations as a search space. Around the same time, Zoph \cite{zoph2016neural} \etal use the a similar search space; however, the authors use more skip connection for the search space.

{\bf Search strategy.} The strategy is used to search an appropriate models in defined search space. There are many approaches to search models such as reinforcement learning \cite{zhong2018practical, zoph2018learning, baker2016designing, zoph2016neural, cai2018efficient} or evolutionay algorithms \cite{real2017large, xie2017genetic, suganuma2017genetic}. 

{\bf Optimization strategy} This strategy support NAS to guide the network search process. To complete this task, the optimization strategy need to evaluate a search model with a training data without training this models. Different methods are used to enhance the performance of this strategy like network morphisms or one-shot models. 
\subsection{Auto-Keras}
\ak is one of the state-of-the-art AutoML system, which has implemented network morphism \cite{chen2015net2net, wei2016network} to reduce the searching time of NAS. Network morphism is a technique to morph a DNN without changing its functionality. Thus, when \ak find out a new model, instead of training that model from the beginning, \ak can use the information from father DNN to reduce the training time. Nevertheless, even though \ak apply network morphism technique, it still takes a lot of GPU computation. Therefore, we desire to use mined DNN models to enhance the performance of \ak.

==> evaluation/RQ6.tex <==
%\begin{table}
%	\centering
%	\caption{Accuracy Ranking}
%	\setlength{\tabcolsep}{3pt}
%	\footnotesize
%
%\begin{tabular}{|c|c|c|c|}
%
%\hline
%
%	\begin{tabular}[c]{@{}c@{}}{\bf Training} \\ {\bf Data}\end{tabular} & \begin{tabular}[c]{@{}c@{}}{\bf Ranking}\end{tabular} & \begin{tabular}[c]{@{}c@{}}{\bf Method} \end{tabular} & \begin{tabular}[c]{@{}c@{}}{\bf Accuracy} \end{tabular}  \\ \hline \hline
%		\multirow{8}{*}{Blood Cell}			&1     	&\manas      				&87.74\%         				\\ \cline{2-4} 
%	&2      &Hand-designed model 1  			&86.78\%	 		 		\\ \cline{2-4} 
%	&3		&Hand-designed model 2        	&85.85\%              		\\ \cline{2-4} 
%	&4      &Hand-designed model 3        	&85.73\%               		\\ \cline{2-4} 
%	&5      &Hand-designed model 4        	&84.40\%           			\\ \cline{2-4} 
%	&6      &Hand-designed model 5	        &83.76\%               		\\ \cline{2-4} 
%	&7      &\ak        				&83.55\%          			\\ \hline \hline
%	
%					
%
%
%%		\multirow{8}{*}{Kannada MNIST}			
%%	&1     	&      		&        				\\ \cline{2-4} 
%%	&2      &  			&	 		 		\\ \cline{2-4} 
%%	&3		&        	&              		\\ \cline{2-4} 
%%	&4      &        	&              		\\ \cline{2-4} 
%%	&5      &        	&          			\\ \cline{2-4} 
%%	&6      &	        &               		\\ \cline{2-4} 
%%	&7      &        	&         			\\ \hline \hline
%	
%	\multirow{7}{*}{Malaria}			&1		&Hand-designed model 1       	&97.50\% 		 		\\ \cline{2-4}  
%	&2      &Hand-designed model 2        	&97.39\%        		\\ \cline{2-4}
%	&3      &\manas						&97.19\%              	\\ \cline{2-4} 
%	&4      &\ak        				&96.64\%               		\\ \cline{2-4} 
%	&5      &Hand-designed model 3        	&95.54\%           			\\ \cline{2-4} 
%	&6      &Hand-designed model 4        	&92.50\%               		\\ \cline{2-4} 
%	&7      &Hand-designed model 5        	&85.00\%          				\\ \hline \hline
%		
%%		\multirow{8}{*}{MNIST}			
%%	&1     	&      		&        				\\ \cline{2-4} 
%%	&2      &  			&	 		 		\\ \cline{2-4} 
%%	&3		&        	&              		\\ \cline{2-4} 
%%	&4      &        	&              		\\ \cline{2-4} 
%%	&5      &        	&          			\\ \cline{2-4} 
%%	&6      &	        &               		\\ \cline{2-4} 
%%	&7      &        	&         			\\ \hline \hline					
%	\multirow{8}{*}{Sign-Digits}			
%	&1     	&\manas       				&100.00\%        				\\ \cline{2-4} 
%	&1      &Handmade model 1 					&100.00\%	 		 		\\ \cline{2-4} 
%	&3		&Handmade model 2        	&99.51\%              		\\ \cline{2-4} 
%	&4      &Handmade model 3        	&99.00\%              		\\ \cline{2-4} 
%	&5      &\ak        				&98.79\%          			\\ \cline{2-4} 
%	&6      &Handmade model 4	        &95.00\%               		\\ \cline{2-4} 
%	&7      &Handmade model 5        	&89.00\%         			\\ \hline 
%	
%
%	
%	 
%										
%%	\multirow{8}{*}{Sign-Language-Digits}&1     &\manas       				&100.00\%         		\\ \cline{2-4} 
%%										&2      &Handmade model 1        	&100.00\%              		\\ \cline{2-4} 
%%										&3      &Handmade model 2       	&99.51\%           			\\ \cline{2-4} 
%%										&4      &Handmade model 3        	&99.00\%               		\\ \cline{2-4} 
%%										&5      &\ak        				&97.08\%           			\\ \cline{2-4}  
%%										&6      &Handmade model 4	        &95.00\%               		\\ \cline{2-4}	
%%										&7		&Handmade model 5 			&89.00\%		 		 \\ \hline
%																			
%\end{tabular}
%	\label{tbl:ranking}
%\end{table}



\begin{table}[]
	\begin{tabular}{|c|c|c|c|c|c|c|c|}
		\hline
			& Blood Cell 			& Fashion & Flower & Ham 	& Malaria  		& SL 	& SD  \\ \hline
		1 	& HD1 (8.66)          	&         &        &   		&    			& \manas (100)      &                                                               \\ \hline
		2 	& \manas (10.18)        &         &        &   		&    			& HD1 (100)     &                                                               \\ \hline
		3 	& HD2 (12.3)           	&         &        &   		&   			& HD2 ()99.51)       &                                                               \\ \hline
		4 	& HD3 (12.7)           	&         &        &   		&    			& HD3 (99.00)      &                                                               \\ \hline
		5 	& \ak (14.07)          	&         &        &   		&    			& \ak (98.70)      &                                                               \\ \hline
		
	\end{tabular}
\end{table}

==> evaluation/results2.tex <==
\begin{figure*}[]
	\includegraphics[width=0.99\textwidth]{images/all.png}
	\caption{Error Rate and MSE of \ak, \om, \tm, and \manas over time}
	\label{fig:results}
\end{figure*}


==> framework/adaptation.tex <==
\subsection{Adaptation System}
\label{sec:adapt}

The adaptation system \circled{4} is used to adapt deep learning models and optimizers from the database into \manas. We store the extracted CNN models in a database as an abstract neural network (AbNN), 
which is an abstract representation of the neural network. 
This representation has the structure as a network where the nodes are API calls, 
and the connections are the order between API calls. 
We use this representation to adapt models and their optimizers into \manas. From each node, we obtain the name of layer and its parameters, which can be converted into an API call. 
Figure \ref{fig:converted} presents an example of AbNN built from an mined model. Notice that
if an activation parameter is implemented as an argument inside a layer, 
we consider that the activation is a separate layer. 

\begin{figure}
	\centering
	\begin{subfigure}[b]{.45\linewidth}
		\begin{lstlisting}[basicstyle=\tiny,numberblanklines=false]
		Conv2D(64, kernel_size = (3, 3),activation='relu',input_shape=(3, 120, 180))
		
		MaxPooling2D(pool_size=(2,2))
		Conv2D(32,                   activation='relu')
		
		MaxPooling2D(pool_size=(2,2))
		Dropout(0.25)
		Flatten()
		Dense(20, activation='softmax')


		SGD(lr=0.01, decay=1e-6) @\label{line:optim}@
\end{lstlisting}
		\caption{Extracted model}
		\label{fig:originalCNN}
	\end{subfigure}
	\begin{subfigure}[b]{.45\linewidth}
		\begin{lstlisting}[basicstyle=\tiny,numberblanklines=false]	
		{'func': 'Conv2D', 'input_shape': [3, 120, 180], 'arg2': 64, 'kernel_size': [3, 3]} @\label{line:example}@
		{'func': 'relu'}
		{'func': 'MaxPool2d', 'pool_size': [2, 2]}
		{'func': 'Conv2D', 'arg1': 64, 'arg2': 32}
		{'func': 'relu'}
		{'func': 'MaxPool2d', 'pool_size': [2, 2]}
		{'func': 'Dropout', 'arg1': 0.25}
		{'func': 'Flatten'}
		{'func': 'linear', 'arg1': 128, 'arg2': 20}
		{'func': 'softmax'}
		
		{'func': 'SGD', 'lr': 0.01, 'decay': 1e-06} @\label{line:optimconvert}@
\end{lstlisting}
		\caption{Abstract Neural Network}
		\label{fig:convertedCNN}
	\end{subfigure}
	\caption{Building an abstraction of neural network from extracted model}
	\vspace{-5mm}
	\label{fig:converted}
\end{figure}




==> framework/benchmark.tex <==
\section{DNN model benchmark}

==> framework/converter.tex <==
\subsection{Adaptation System}
\label{sec:adapt}
Adaptation system \circled{4} is used to adapt deep learning models and optimizers from the database into \manas. Two main steps of adaptation system is model adaptation and training adaptation.
%\input{algorithms/adapt.tex}
%\subsubsection{ Model Adaptation} 

Model adaptation help \manas to convert ANN into \manas' models. Adapting the ANN has two steps, which are converting the layers and converting the connections. To adapt the a model's layer, we need to adapt correctly the layer type and it's parameters. The layer type can be obtained from the first argument of each ANN's layer. For the positional arguments, which are may not be not set the parameter,

\manas use not only model structures of deep learning developers but also their optimizers. In fact, it is challenging to pick a suitable optimizer. The deep learning developers sometimes have to retrain models multiple times to find out a good optimizer. Thus, we utilize their work to increase the performance of \manas. Particularly, instead of using a constant default optimizer like \ak, \manas mine the optimizer from repositories and use it based on chosen candidate models. In other words, whenever \manas trains a candidate model, it will use the model's optimizer. If a model either does not include an optimizer or an unsupported optimizer, we will use the \ak's default optimizer. 

%Thus, after mining the models, we have converted them into ANN, which represents both the layer and the connection. The different layer needs different kinds of required parameters. For example, the convolution layer has four requirement parameters, which include the input channel, output channel, kernel size, and strides. For the input layer and output layer, we have to modify the input size and output channel of the models to be compatible with the training data. In other words, the candidate model uses the input layer and the output channel of the user instead of its original values. Furthermore, \manas uses \code{output\_node} to create the connection of each layer with the other layers.

%\subsubsection{ Training Adaptation} 





==> framework/trainingadaptation.tex <==
\section{Training Adaptation}



(NOTE: explain why not search the model from the first times. Example)

(NOTE: process to change the optimizer. Image. example)
%We modify the optimizer of \manas based on the mined common optimizer. We, first of all, collect all optimizers API of Pytorch which are Adadelta, Adagrad, Adam, SparseAdam, Adamax, ASGD, LBFGS, RMSprop, Rprop, SGD. Then, using mined Python files from the model mining technique, we use CFG to obtain the Python files which contain these optimizers API. Table \ref{optimizerfrequence} show the frequency of each optimizer from mined Python codes from repositories.
%
%
%
%The table \ref{optimizerfrequence} show that the most used optimizer are Adam, SGD, and RMSprop; therefore, we select them as good optimizer to modify \manas. With each optimizer, we have four most common value of learning rates, which are 0.1, 0.01, 0.001, 0.0001. We use these optimizers and the learning rates on the candidate models and train them in 2 hours on a specific dataset. Overall, we will select the set of the optimizer, learning rate, and model architecture, which has the best accuracy for the final search. 

==> motivation.tex <==
\section{motivation}
\subsection{Initial models of AutoKeras}
We were fascinated by \ak when we read the paper \cite{jin2018efficient}; therefore, we desire to explore how does \ak work. At the beggining \ak will create some inital ML models. Then, \ak train these models on input data and select the best one. \ak bases on the result from the selection model and uses reinforce learning modify the selection model. However, \ak only uses some constant initial models architecture for all kinds of dataset. Thus, we was wondering that can we improve the performance of \ak on one kind of dataset, if we choose a better models and make them become initial models of \ak. Moreover, when we learn how to use \ak, we also realize that \ak did really good work on MNIST, Cifar10, Fashion. However, the results of \ak on the other datasets are not good. For example, when we run \ak on "Chest X-Ray Pneumonia" dataset \footnote{\url{https://www.kaggle.com/paultimothymooney/chest-xray-pneumonia}} dataset, \ak only achieve the accuracy ..,..,.. after 4 hours, 8 hours, 16 hours, respectively. Therefore, we try to pick models from a good reposistories on \gh and make it become the initial results of \ak. After 4 hours, 8 hours, and 16 hours of training, we have the result like the "image". \footnote{\url{https://stackoverflow.com/questions/37213388/keras-accuracy-does-not-change}}

The results shows that AutoKeras with new initial models give the better results than both the original AutoKeras and the best model from Kaggle for "Chest X-Ray Pneumonia" dataset. 
\end{motivation}

==> tables/clustering.tex <==
\begin{table*}[]
	\centering
	\caption{Manas' models vs hand-made models}
\resizebox{\textwidth}{!}{%
	\begin{tabular}{cccccccccccccccccccccccccc}
		\hline
		\multicolumn{2}{c}{Blood Cell}                                &  & \multicolumn{2}{c}{Breast Cancer}                             &  & \multicolumn{2}{c}{Chest X-Ray}                               &  & \multicolumn{2}{c}{Flower}                                    &  & \multicolumn{2}{c}{IIC}                                       &  & \multicolumn{2}{c}{Malaria}                                   &  & \multicolumn{2}{c}{MNIST: HAM}                                &  & \multicolumn{2}{c}{SD}                               &  & \multicolumn{2}{c}{SL}                             \\ \cline{1-2} \cline{4-5} \cline{7-8} \cline{10-11} \cline{13-14} \cline{16-17} \cline{19-20} \cline{22-23} \cline{25-26} 
		Models & \begin{tabular}[c]{@{}c@{}}Error\\ Rate\end{tabular} &  & Models & \begin{tabular}[c]{@{}c@{}}Error\\ Rate\end{tabular} &  & Models & \begin{tabular}[c]{@{}c@{}}Error\\ Rate\end{tabular} &  & Models & \begin{tabular}[c]{@{}c@{}}Error\\ Rate\end{tabular} &  & Models & \begin{tabular}[c]{@{}c@{}}Error\\ Rate\end{tabular} &  & Models & \begin{tabular}[c]{@{}c@{}}Error\\ Rate\end{tabular} &  & Models & \begin{tabular}[c]{@{}c@{}}Error\\ Rate\end{tabular} &  & Models & \begin{tabular}[c]{@{}c@{}}Error\\ Rate\end{tabular} &  & Models & \begin{tabular}[c]{@{}c@{}}Error\\ Rate\end{tabular} \\ \hline
		HM1 \cite{bloodcell1} & 8.7                                                  &  & HM1 \cite{breastcancer1}   & 5.9                                                  &  & MN     & 7.4                                                  &  & HM1 \cite{flower1}    & 6.7                                                  &  & HM1 \cite{IIC1}    & 8.4                                                  &  & MN     & 1.6                                                  &  & HM1 \cite{ham1}   &  9.8                                                   &  & MN     & 0.0                                                  &  & MN     & 0.0                                                  \\
		MN     & 10.0                                                 &  & HM2 \cite{breastcancer2}    & 6.0                                                  &  & HM1 \cite{xray1}    & 7.4                                                  &  & HM2 \cite{flower2}   & 11.9                                                 &  & HM2 \cite{IIC2}   & 8.5                                                  &  & AK     & 2.3                                                  &  & HM2 \cite{ham2}    & 18.8                                                     &  & HM1 \cite{sd1}   & 0.0                                                  &  & AK     &  0.0                                                  \\
		HM2 \cite{bloodcell2}    & 12.3                                                 &  & MN     & 6.9                                                  &  & HM2 \cite{xray2}     & 9.8                                                  &  & MN     & 12.8                                                 &  & MN     & 8.6                                                  &  & HM1 \cite{malaria1}    & 2.5                                                  &  & MN    & 20.3                                                    &  & AK     &  0.5                                                  &  & HM1 \cite{sl1}   & 0.0                                                  \\
		HM3 \cite{bloodcell3}   & 14.3                                                &  & AK     & 6.9                                                  &  & HM3 \cite{xray3}    & 10.3                                                 &  & AK     & 14.6                                                 &  & AK     & 8.9                                                  &  & HM2 \cite{malaria2}    & 4.0                                                  &  & AK     & 20.6                                                    &  & HM2 \cite{sd1}   & 1.0                                                  &  & HM2 \cite{sl2}  & 0.3                                                  \\
		AK     & 18.9                                                 &  & HM3 \cite{breastcancer3}    & 9.1                                                  &  & AK     & 11.5                                                 &  & HM3 \cite{flower3}   & 17.3                                                 &  & HM3 \cite{IIC3}    & 9.0                                                  &  & HM3 \cite{malaria3}   & 4.5                                                  &  & HM3 \cite{ham3}   & 21.0                                                     &  & HM3 \cite{sd1}    & 2.4                                                  &  & HM3 \cite{sl3}    & 0.5                                                  \\ \hline
	\end{tabular}%
}
	\label{tbl:mn vs hm}
	\centering
\end{table*}

%	\setlength{\tabcolsep}{1.0pt}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{longtable}
% Note: It may be necessary to compile the document several times to get a multi-page table to line up properly
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
%\begin{table*}[]
%	\resizebox{\textwidth}{!}{%
%		\begin{tabular}{ccccccccccc}
%			\hline
%			\multirow{2}{*}{Time} & \multirow{2}{*}{Data} & \begin{tabular}[c]{@{}c@{}}Error Rate \\ (\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Depth \\ (layers)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Param \# \\ (million)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Speed \\ (epoch/mins)\end{tabular} & \multirow{2}{*}{Data} & \begin{tabular}[c]{@{}c@{}}Error Rate \\ (\%)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Depth \\ (layers)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Param \# \\ (million)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Speed \\ (epoch/mins)\end{tabular} \\ \cline{3-6} \cline{8-11} 
%			&                       & \multicolumn{4}{c}{TM$|$OM$|$MN$|$AK}                                                                                                                                                                                                                  &                       & \multicolumn{4}{c}{TM$|$OM$|$MN$|$AK}                                                                                                                                                                                                                  \\ \hline
%			2h                    & \multirow{10}{*}{BC}  
%			&  00.00$|$00.00$|$00.00$|$00.00                                                          
%			&  00.00$|$00.00$|$00.00$|$00.00                                                          
%			&  00.00$|$00.00$|$00.00$|$00.00                                                              &  00.00$|$00.00$|$00.00$|$00.00                                                              
%			& \multirow{10}{*}{SL}  
%			&  00.00$|$00.00$|$00.00$|$00.00                                                           
%			&  00.00$|$00.00$|$00.00$|$00.00                                                          
%			&  00.00$|$00.00$|$00.00$|$00.00                                                              &  00.00$|$00.00$|$00.00$|$00.00                                                              \\
%			4h                    &                       &  00.00$|$00.00$|$00.00$|$00.00                                                          
%			&  00.00$|$00.00$|$00.00$|$00.00                                                          
%			&  00.00$|$00.00$|$00.00$|$00.00                                                              &  00.00$|$00.00$|$00.00$|$00.00                                                              
%			&   
%			&  00.00$|$00.00$|$00.00$|$00.00                                                           
%			&  00.00$|$00.00$|$00.00$|$00.00                                                          
%			&  00.00$|$00.00$|$00.00$|$00.00                                                              &  00.00$|$00.00$|$00.00$|$00.00                                                                 \\
%			6h                    &                       &  00.00$|$00.00$|$00.00$|$00.00                                                          
%			&  00.00$|$00.00$|$00.00$|$00.00                                                          
%			&  00.00$|$00.00$|$00.00$|$00.00                                                              &  00.00$|$00.00$|$00.00$|$00.00                                                              
%			&   
%			&  00.00$|$00.00$|$00.00$|$00.00                                                           
%			&  00.00$|$00.00$|$00.00$|$00.00                                                          
%			&  00.00$|$00.00$|$00.00$|$00.00                                                              &  00.00$|$00.00$|$00.00$|$00.00                                                                 \\
%			8h                    &                       &  00.00$|$00.00$|$00.00$|$00.00                                                          
%			&  00.00$|$00.00$|$00.00$|$00.00                                                          
%			&  00.00$|$00.00$|$00.00$|$00.00                                                              &  00.00$|$00.00$|$00.00$|$00.00                                                              
%			&   
%			&  00.00$|$00.00$|$00.00$|$00.00                                                           
%			&  00.00$|$00.00$|$00.00$|$00.00                                                          
%			&  00.00$|$00.00$|$00.00$|$00.00                                                              &  00.00$|$00.00$|$00.00$|$00.00                                                                 \\
%			10h                   &                       &  00.00$|$00.00$|$00.00$|$00.00                                                          
%			&  00.00$|$00.00$|$00.00$|$00.00                                                          
%			&  00.00$|$00.00$|$00.00$|$00.00                                                              &  00.00$|$00.00$|$00.00$|$00.00                                                              
%			&   
%			&  00.00$|$00.00$|$00.00$|$00.00                                                           
%			&  00.00$|$00.00$|$00.00$|$00.00                                                          
%			&  00.00$|$00.00$|$00.00$|$00.00                                                              &  00.00$|$00.00$|$00.00$|$00.00                                                                 \\
%			12h                   &                       &  00.00$|$00.00$|$00.00$|$00.00                                                          
%			&  00.00$|$00.00$|$00.00$|$00.00                                                          
%			&  00.00$|$00.00$|$00.00$|$00.00                                                              &  00.00$|$00.00$|$00.00$|$00.00                                                              
%			&   
%			&  00.00$|$00.00$|$00.00$|$00.00                                                           
%			&  00.00$|$00.00$|$00.00$|$00.00                                                          
%			&  00.00$|$00.00$|$00.00$|$00.00                                                              &  00.00$|$00.00$|$00.00$|$00.00                                                                 \\
%			14h                   &                       &  00.00$|$00.00$|$00.00$|$00.00                                                          
%			&  00.00$|$00.00$|$00.00$|$00.00                                                          
%			&  00.00$|$00.00$|$00.00$|$00.00                                                              &  00.00$|$00.00$|$00.00$|$00.00                                                              
%			&   
%			&  00.00$|$00.00$|$00.00$|$00.00                                                           
%			&  00.00$|$00.00$|$00.00$|$00.00                                                          
%			&  00.00$|$00.00$|$00.00$|$00.00                                                              &  00.00$|$00.00$|$00.00$|$00.00                                                                 \\
%			16h                   &                       &  00.00$|$00.00$|$00.00$|$00.00                                                          
%			&  00.00$|$00.00$|$00.00$|$00.00                                                          
%			&  00.00$|$00.00$|$00.00$|$00.00                                                              &  00.00$|$00.00$|$00.00$|$00.00                                                              
%			&  
%			&  00.00$|$00.00$|$00.00$|$00.00                                                           
%			&  00.00$|$00.00$|$00.00$|$00.00                                                          
%			&  00.00$|$00.00$|$00.00$|$00.00                                                              &  00.00$|$00.00$|$00.00$|$00.00                                                                 \\
%			18h                   &                       &  00.00$|$00.00$|$00.00$|$00.00                                                          
%			&  00.00$|$00.00$|$00.00$|$00.00                                                          
%			&  00.00$|$00.00$|$00.00$|$00.00                                                              &  00.00$|$00.00$|$00.00$|$00.00                                                              
%			&   
%			&  00.00$|$00.00$|$00.00$|$00.00                                                           
%			&  00.00$|$00.00$|$00.00$|$00.00                                                          
%			&  00.00$|$00.00$|$00.00$|$00.00                                                              &  00.00$|$00.00$|$00.00$|$00.00                                                                 \\
%			20h                   &                       &  00.00$|$00.00$|$00.00$|$00.00                                                          
%			&  00.00$|$00.00$|$00.00$|$00.00                                                          
%			&  00.00$|$00.00$|$00.00$|$00.00                                                              &  00.00$|$00.00$|$00.00$|$00.00                                                              
%			&  
%			&  00.00$|$00.00$|$00.00$|$00.00                                                           
%			&  00.00$|$00.00$|$00.00$|$00.00                                                          
%			&  00.00$|$00.00$|$00.00$|$00.00                                                              &  00.00$|$00.00$|$00.00$|$00.00                                                                \\ \hline
%		\end{tabular}%
%	}
%\end{table*}

==> tables/evaRegression.tex <==
\begin{table}[H]
	\centering
	\caption{Evaluation of Regression Problem}
	\label{tbl:regression}
	\setlength{\tabcolsep}{4pt}
	\footnotesize
	\renewcommand{\arraystretch}{1}
	\begin{tabular}{|c|c|c|c|c|c|c|}
		\hline
		\rowcolor{gray!50}
		\begin{tabular}[c]{@{}c@{}}Training \\ Data\end{tabular} & \begin{tabular}[c]{@{}c@{}}Time \\ (hours)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Original \\ \ak\\ (AK)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Handmade \\ Model\end{tabular} & \begin{tabular}[c]{@{}c@{}}AK with \\ MM\end{tabular} & \begin{tabular}[c]{@{}c@{}}AK with \\ TMM\end{tabular} & \begin{tabular}[c]{@{}c@{}}AK with \\  TMM \\ and MO\end{tabular} \\ \hline
		\multirow{8}{*}{Malaria}	&1		&		&		&		&		& 		\\ \cline{2-7} 
									&2     	&       	&       &      	&       &  		\\ \cline{2-7} 
									&3      &        &       &        &       &        		\\ \cline{2-7} 
									&4      &        &       &        &       &         		\\ \cline{2-7} 
									&5      &        &       &        &       &     			\\ \cline{2-7} 
									&6      &        &       &        &       &        		\\ \cline{2-7} 
									&7      &        &       &        &       &   				\\ \cline{2-7} 
									&8      &        &       &        &       &          		\\ \hline
		\multirow{8}{*}{Chest X-ray}&1		&		&		&		&		& 		\\ \cline{2-7} 
									&2     	&       	&       &      	&       &  		\\ \cline{2-7} 
									&3      &        &       &        &       &        		\\ \cline{2-7} 
									&4      &        &       &       &       &         		\\ \cline{2-7} 
									&5      &        &       &        &       &     			\\ \cline{2-7} 
									&6      &        &       &        &       &        		\\ \cline{2-7} 
									&7      &        &       &        &       &   				\\ \cline{2-7} 
									&8      &        &       &        &       &          		\\ \hline
		\multirow{8}{*}{Dogs vs Cats}		&1		&		&		&		&		& 		\\ \cline{2-7} 
									&2     	&       	&       &      	&       &  		\\ \cline{2-7} 
									&3      &        &       &        &       &        		\\ \cline{2-7} 
									&4      &        &       &       &       &         		\\ \cline{2-7} 
									&5      &        &       &        &       &     			\\ \cline{2-7} 
									&6      &        &       &        &       &        		\\ \cline{2-7} 
									&7      &        &       &        &       &   				\\ \cline{2-7} 
									&8      &        &       &        &       &          		\\ \hline
	\end{tabular}
	\label{tbl:evaRegression}
\end{table}



==> tables/inout.tex <==
%\begin{table}[H]
%	\centering
%	\caption{Input Size vs Output Channel.}
%	\setlength{\tabcolsep}{0.5pt}
%	\footnotesize
%	\begin{tabular}{|c|c|c|}
%		\hline
%		\rowcolor{gray!50}
%		Data 			& Output Channel    & Input Size \\ \hline   %& M13   & M14   
%		Blood Cell 		& 87.74\%|00:13:39
%						& 87.74\%|00:13:39  \\ \hline % & 0.960 & 0.959
%		Malaria    		& 96.73\%|02:36:42  
%						& 97.19\%|1:02:34 \\ \hline% 0.518 & 0.479 
%		Chest X-ray     & 83.47\%|0:20:52 
%						& 86.06\%|0:24:59  \\ \hline% 0.518 & 0.479 
%	\end{tabular}
%	\label{tbl:inout}
%\end{table}

\begin{table}[ht]
	\centering
	\caption{Input Size vs Output Channel.}
	\setlength{\tabcolsep}{1.5pt}	
	\footnotesize
	
	\begin{tabular}{|c|c|c|c|c|}
		\hline
		\textbf{Data} & \textbf{Output Channel} & \textbf{Input Size} \\ \hline \hline
		Blood Cell    & 87.74\%                 & 87.74\%             \\ \hline
		Fashion MNIST & 92.71\%                   & 92.71\%           \\ \hline
		Malaria       & 96.73\%                 & 97.19\%                      \\ \hline
		MNIST         & 99.45\%                      &  99.45\%                   \\ \hline
		Sign-Digits    & 100.0\%                 & 100.0\%                    \\ \hline
	\end{tabular}
	\label{tbl:inout}
\end{table}



==> tables/motivateAKcell.tex <==
%\begin{table}[H]
%	\centering
%	\caption{\ak vs \manas on Blood Cell dataset.}
%	\setlength{\tabcolsep}{1pt}
%	\footnotesize
%	\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|}
%		\hline
%		\rowcolor{gray!50}
%\multicolumn{3}{|c|}{Error Rate(\%)}    & \multicolumn{3}{c|}{Model Depth}  & \multicolumn{3}{c|}{Model Width} &\multicolumn{3}{c|}{Time/epoch} \\ \hline
%\ak & \manas & \% decrease & \ak & \manas & \% decrease & \ak & \manas & \% decrease & \ak & \manas & \% decrease \\ \hline
%14.08              & 10.26                 & 27.13       & 21                 & 08                    & 61.90       & 11M                & 0.176M                & 98.4        & 75'                & 60'                   & 20          \\ \hline
%\end{tabular}  
%
%	\label{tbl:error}
%\end{table}

\begin{table}[H]
	\centering
	\caption{\ak vs \manas on Blood Cell dataset.}
	\setlength{\tabcolsep}{1pt}
	\footnotesize
	\begin{tabular}{|c|c|c|c|c|}
		\hline
		\rowcolor{gray!50}
		            & Error Rate(\%) & Model Depth & Model Width & Time/epoch \\ \hline
		\ak          & 14.08 \%          & 21 layers        & 11M         & 75'        \\ \hline
		\manas       & 10.26 \%         & 08 layers         & 0.176M      & 60'        \\ \hline
		Percentage Decrease & 27.13\%          & 61.90\%       & 98.40\%        & 20.00\%         \\ \hline
	\end{tabular}  
	
	\label{tbl:avm}
\end{table}

==> tables/motivateAKxray.tex <==
%\begin{table}[ht]
%	\centering
%	\caption{2 hours of \ak on Chest X-Ray Pneumonia.}
%	\setlength{\tabcolsep}{4.5pt}
%	\footnotesize
%	\begin{tabular}{|c|c|c|}
%		\hline
%		\rowcolor{gray!50}
%		Model ID & M1     & M2     \\ \hline
%		Accuracy               & 0.92      	 & 0.91      \\ \hline
%		Loss                   & 0.77 		 & 0.85 \\ \hline
%	\end{tabular}
%	\label{tbl:AKXray2hour}
%\end{table}

\begin{table}[ht]
	\centering
	\caption{2 hours of \ak on Chest X-Ray Pneumonia.}
	\setlength{\tabcolsep}{1.5pt}
	\footnotesize
	\begin{tcolorbox}[tabularx={X||Y|Y},
		lifted shadow={1mm}{-2mm}{3mm}{0.1mm}{black!50!white},
		,text width=150pt]
		%\rowcolor{darksalmon}
		Model ID 	& M1     & M2       \\\hline\hline
		Accuracy   	& 0.92 & 0.91  		\\\hline
		Loss 		& 0.77 & 0.85  		
	\end{tcolorbox}
	\label{tbl:AKXray2hour}
\end{table}
%\begin{table}[ht]
%	\centering
%	\caption{2 hours of \ak on Chest X-Ray Pneumonia.}
%	\begin{tcolorbox}[tab2,tabularx={X||Y|Y|Y|Y||Y}]
%		
%		Group & One     & Two     & Three    & Four     & Sum      \\\hline\hline
%		Red   & 1000.00 & 2000.00 &  3000.00 &  4000.00 & 10000.00 \\\hline
%		Green & 2000.00 & 3000.00 &  4000.00 &  5000.00 & 14000.00 \\\hline
%		Blue  & 3000.00 & 4000.00 &  5000.00 &  6000.00 & 18000.00 \\\hline\hline
%		Sum   & 6000.00 & 9000.00 & 12000.00 & 15000.00 & 42000.00
%	\end{tcolorbox}
%	\label{tbl:AKXray2hour}
%\end{table}

==> tables/motivateComplexity.tex <==
\begin{table}[H]
	\centering
	\caption{\ak vs \manas on Blood Cell dataset.}
	\setlength{\tabcolsep}{1pt}
	\footnotesize
	\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
		\hline
		\rowcolor{gray!50}
		Hours & 1    & 2    & 3    & 4    & 5    & 6    & 7    & 8   \\ \hline   %& M13   & M14   
		\ak & 14.08 & 14.08 & 14.08 & 14.08 & 14.08 & 14.08 & 14.08 & 14.08  \\ \hline % & 0.960 & 0.959
		\manas     & 10.26 & 10.26 & 10.26 & 10.26 & 10.26 & 10.26 & 10.26 & 10.26 \\ \hline% 0.518 & 0.479 
		Decrease percentage     &  &  &  &  &  &  &  & \\ \hline
	\end{tabular}
	\label{tbl:complex}
\end{table}

==> tables/motivateModAKxray.tex <==
\begin{table}[ht]
	\centering
	\caption{2 hours of \ak with mined default models on Chest X-Ray Pneumonia dataset.}
	\setlength{\tabcolsep}{4.5pt}
	\footnotesize
	\begin{tabular}{|c|c|c|c|c|c|c|}
		\hline
		\rowcolor{gray!50}
		Model ID & M1    & M2       & M3     & M4     & M5     	& M6     \\ \hline
		Accuracy               & 0.94      	& 0.83     	 	& 0.94        & 0.91        & 0.95      	& 0.97       \\ \hline
		Loss                   & 0.65 		& 10.14 		& 0.75 		  & 2.90 		& 0.50 			& 0.36 \\ \hline
	\end{tabular}
	\label{tbl:toolXray2hour}
\end{table}


==> tables/thresholdClassification.tex <==
%\begin{table}[H]
%	\centering
%	\caption{Evaluation for Transformation Models}
%	\label{tbl:evalTrans}
%	\setlength{\tabcolsep}{3pt}
%	\footnotesize
%	\renewcommand{\arraystretch}{1}
%	\begin{tabular}{|c|c|c|c|c|c|}
%		\hline
%		\rowcolor{gray!50}
%		\multicolumn{1}{|c|}{Training Data} & \multicolumn{1}{|c|}{\manas 1} & \multicolumn{1}{c|}{\manas 2} 
%											& \multicolumn{1}{c|}{\manas 3} & \multicolumn{1}{c|}{\ak}   \\ \hline
%		\multicolumn{1}{|c|}{Blood Cell}	&\begin{tabular}[c]{@{}c@{}}83.55\%\\02:01:55\end{tabular} 
%											&\begin{tabular}[c]{@{}c@{}}74.47\%\\ 00:39:21\end{tabular}    
%										    &\begin{tabular}[c]{@{}c@{}}83.35\%\\ 00:58:54\end{tabular}     			
%										    &\begin{tabular}[c]{@{}c@{}}87.74\%\\ 00:13:39\end{tabular}\\ \hline
%		\multicolumn{1}{|c|}{Malaria}		&\begin{tabular}[c]{@{}c@{}}96.64\%\\ 00:35:19\end{tabular}   
%											&\begin{tabular}[c]{@{}c@{}}96.75\%\\ 01:09:43\end{tabular}    
%											&\begin{tabular}[c]{@{}c@{}}83.35\%\\ 00:58:54\end{tabular}     			
%											&\begin{tabular}[c]{@{}c@{}}97.19\%\\ 01:02:33\end{tabular}\\ \hline
%											&                                &                               &                               &     						\\ \hline
%	\end{tabular}
%
%\end{table}

%\begin{table}[ht]
%	\centering
%	\caption{Evaluation of Classification Problem}
%	\setlength{\tabcolsep}{4pt}
%	\footnotesize
%	\renewcommand{\arraystretch}{1}
%	\begin{tabular}{|c|c|c|c|c|c|}
%		\hline
%		\rowcolor{gray!50}
%		\begin{tabular}[c]{@{}c@{}}Training \\ Data\end{tabular} & \begin{tabular}[c]{@{}c@{}}Searching \\Time (hrs)\end{tabular} & \ak
%		& \manas1 & \manas2 & \manas3 \\ \hline
%		\multirow{8}{*}{Malaria}	&1		&\begin{tabular}[c]{@{}c@{}}96.12\%\\ 00:32:58\end{tabular}						&\begin{tabular}[c]{@{}c@{}}97.17\%\\ 01:01:41\end{tabular}		
%		&						&\begin{tabular}[c]{@{}c@{}}97.53\%\\ 01:59:19\end{tabular}		\\ \cline{2-6} 
%		
%		&2  	&\begin{tabular}[c]{@{}c@{}}96.39\%\\ 00:36:58\end{tabular}						&\begin{tabular}[c]{@{}c@{}}97.17\%\\ 01:01:41\end{tabular}      	
%		&       				&\begin{tabular}[c]{@{}c@{}}97.53\%\\ 01:59:19\end{tabular}  		\\ \cline{2-6}  
%		
%		&3  	&\begin{tabular}[c]{@{}c@{}}96.64\%\\ 00:35:19\end{tabular}						&\begin{tabular}[c]{@{}c@{}}97.20\%\\ 01:01:39\end{tabular}        
%		&      	 				&\begin{tabular}[c]{@{}c@{}}97.26\%\\ 01:30:38\end{tabular}        		\\ \cline{2-6}  
%		
%		&4  	&\begin{tabular}[c]{@{}c@{}}96.64\%\\ 00:35:19\end{tabular}						&\begin{tabular}[c]{@{}c@{}}97.06\%\\ 01:09:59\end{tabular}        
%		&       &\begin{tabular}[c]{@{}c@{}}97.30\%\\ 01:11:49\end{tabular}         		\\ \cline{2-6}  
%		
%		&5  	&\begin{tabular}[c]{@{}c@{}}96.64\%\\ 00:35:19\end{tabular}						&\begin{tabular}[c]{@{}c@{}}97.06\%\\ 01:09:59\end{tabular}        
%		&       &\begin{tabular}[c]{@{}c@{}}97.30\%\\ 01:11:49\end{tabular}     			\\ \cline{2-6}  
%		
%		&6  	&\begin{tabular}[c]{@{}c@{}}96.64\%\\ 00:35:19\end{tabular}						&\begin{tabular}[c]{@{}c@{}}97.06\%\\ 01:09:59\end{tabular}        
%		&       &\begin{tabular}[c]{@{}c@{}}97.30\%\\ 01:11:49\end{tabular}        		\\ \cline{2-6}  
%		
%		&7  	&\begin{tabular}[c]{@{}c@{}}96.64\%\\ 00:35:19\end{tabular}						&\begin{tabular}[c]{@{}c@{}}97.06\%\\ 01:09:59\end{tabular}        
%		&       &\begin{tabular}[c]{@{}c@{}}97.30\%\\ 01:11:49\end{tabular}   				\\ \cline{2-6}  
%		
%		&8  	&\begin{tabular}[c]{@{}c@{}}96.64\%\\ 00:35:19\end{tabular}						&\begin{tabular}[c]{@{}c@{}}97.06\%\\ 01:09:59\end{tabular}        
%		&       &\begin{tabular}[c]{@{}c@{}}97.30\%\\ 01:11:49\end{tabular}          		\\ \hline
%		\multirow{8}{*}{Chest X-ray}&1	&\begin{tabular}[c]{@{}c@{}}96.30\%\\ 01:12:56\end{tabular}	&\begin{tabular}[c]{@{}c@{}}99.32\%\\ 00:57:32\end{tabular}		
%		&		& 		\\ \cline{2-6}  
%		
%		&2  &\begin{tabular}[c]{@{}c@{}}96.30\%\\ 01:12:56\end{tabular}	&\begin{tabular}[c]{@{}c@{}}99.46\%\\ 00:44:16\end{tabular}      	
%		&       &  		\\ \cline{2-6}  
%		
%		&3  &\begin{tabular}[c]{@{}c@{}}96.17\%\\ 01:17:00\end{tabular}	&\begin{tabular}[c]{@{}c@{}}99.46\%\\ 00:44:16\end{tabular}        
%		&       &        		\\ \cline{2-6}  
%		
%		&4  &\begin{tabular}[c]{@{}c@{}}96.01\%\\ 01:20:54\end{tabular}	&\begin{tabular}[c]{@{}c@{}}99.46\%\\ 00:44:16\end{tabular}       	
%		&       &         		\\ \cline{2-6}  
%		
%		&5  &\begin{tabular}[c]{@{}c@{}}96.01\%\\ 01:20:54\end{tabular}	&\begin{tabular}[c]{@{}c@{}}99.43\%\\ 00:58:55\end{tabular}        
%		&       &     			\\ \cline{2-6}  
%		
%		&6  &\begin{tabular}[c]{@{}c@{}}96.01\%\\ 01:20:54\end{tabular}	&\begin{tabular}[c]{@{}c@{}}99.60\%\\ 01:16:25\end{tabular}        
%		&       &        		\\ \cline{2-6}  
%		
%		&7  &\begin{tabular}[c]{@{}c@{}}96.01\%\\ 01:20:54\end{tabular}	&\begin{tabular}[c]{@{}c@{}}99.60\%\\ 01:16:25\end{tabular}        
%		&       &   				\\ \cline{2-6}  
%		
%		&8  &\begin{tabular}[c]{@{}c@{}}96.01\%\\ 01:20:54\end{tabular}	&\begin{tabular}[c]{@{}c@{}}99.60\%\\ 01:16:25\end{tabular}        
%		&       &          		\\ \hline
%		\multirow{8}{*}{Dogs vs Cats}		&1		&\begin{tabular}[c]{@{}c@{}}85.44\%\\ 00:48:52\end{tabular}	&\begin{tabular}[c]{@{}c@{}}92.64\%\\ 00:31:11\end{tabular}		
%		&		& 		\\ \cline{2-6}  
%		
%		&2  	&\begin{tabular}[c]{@{}c@{}}89.10\%\\ 00:52:29\end{tabular}	&\begin{tabular}[c]{@{}c@{}}92.48\%\\ 00:31:30\end{tabular}      	
%		&       &  		\\ \cline{2-6}  
%		
%		&3  	&\begin{tabular}[c]{@{}c@{}}91.24\%\\ 01:51:09\end{tabular}	&\begin{tabular}[c]{@{}c@{}}92.40\%\\ 00:32:30\end{tabular}        
%		&       &        		\\ \cline{2-6}  
%		
%		&4  	&\begin{tabular}[c]{@{}c@{}}91.24\%\\ 01:51:09\end{tabular}	&\begin{tabular}[c]{@{}c@{}}92.40\%\\ 00:32:30\end{tabular}       	
%		&       &         		\\ \cline{2-6}  
%		
%		&5  	&\begin{tabular}[c]{@{}c@{}}91.22\%\\ 02:04:16\end{tabular}	&\begin{tabular}[c]{@{}c@{}}92.54\%\\ 00:34:57\end{tabular}        
%		&       &     			\\ \cline{2-6}  
%		
%		&6  	&\begin{tabular}[c]{@{}c@{}}91.22\%\\ 02:04:16\end{tabular}	&\begin{tabular}[c]{@{}c@{}}92.54\%\\ 00:34:57\end{tabular}        
%		&       &        		\\ \cline{2-6}  
%		
%		&7  	&\begin{tabular}[c]{@{}c@{}}91.22\%\\ 02:04:16\end{tabular}	&\begin{tabular}[c]{@{}c@{}}92.54\%\\ 00:34:57\end{tabular}        
%		&       &   				\\ \cline{2-6}  
%		
%		&8  	&\begin{tabular}[c]{@{}c@{}}91.22\%\\ 02:04:16\end{tabular}	&\begin{tabular}[c]{@{}c@{}}92.54\%\\ 00:34:57\end{tabular}        
%		&       &          		\\ \hline
%	\end{tabular}
%	\label{tbl:evaClassification}
%\end{table}

==> tables/thresholdRegression.tex <==
\begin{table}[H]
	\centering
	\caption{Threshold Evaluation for Regression Problem}
	\setlength{\tabcolsep}{3pt}
	\footnotesize
	\renewcommand{\arraystretch}{1}
	\begin{tabular}{|l|l|l|l|l|l|}
		\hline
		\rowcolor{gray!50}
		\multicolumn{1}{|c|}{Training Data} & \multicolumn{1}{|c|}{Model ID} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}MSE and \\ Loss Threshold\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}AK with\\ MM\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}AK with\\ TMM\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}AK with TMM\\ and MO\end{tabular}} \\ \hline
		&                                                                                             &                                                                                    &                                                                                    &      &                                                                                           \\ \hline
		&                                                                                             &                                                                                    &                                                                                      &    &                                                                                           \\ \hline
		&                                                                                             &                                                                                    &                                                                                     &     &                                                                                           \\ \hline
	\end{tabular}
	\label{tbl:evaThresholdRegression}
\end{table}

